The Limits of Transfer Reinforcement Learning with Latent Low-rank Structure

Many reinforcement learning (RL) algorithms are too costly to use in practice due to the large sizes $S, A$ of the problem's state and action space. To resolve this issue, we study transfer RL with latent low rank structure. We consider the problem of transferring a latent low rank representation when the source and target MDPs have transition kernels with Tucker rank $(S , d, A )$, $(S , S , d), (d, S, A )$, or $(d , d , d )$. In each setting, we introduce the transfer-ability coefficient $\alpha$ that measures the difficulty of representational transfer. Our algorithm learns latent representations in each source MDP and then exploits the linear structure to remove the dependence on $S, A $, or $S A$ in the target MDP regret bound. We complement our positive results with information theoretic lower bounds that show our algorithms (excluding the ($d, d, d$) setting) are minimax-optimal with respect to $\alpha$.

==> content/abstract.tex <==
Many reinforcement learning (RL) algorithms are too costly to use in practice due to the size of the problem's state space $S$ or action space $A$. To resolve this issue, we study transfer RL with latent low rank structure; specifically, we consider the settings in which the source and target MDPs have transition kernels with Tucker rank $(|S|, d, |A|)$, $(|S|, |S|, d), (d, |S|, |A|)$, or $(|S|, d, d)$. In each setting, we introduce the transfer-ability coefficient $\alpha$ that measures the difficulty of performing transfer learning. Our algorithm first learns latent representations in each source MDP and then use linear MDP techniques to remove the dependence on $|S|, |A|$, or $|S||A|$ in the target MDP's regret bound. We complement our positive results with information theoretic lower bounds that show our algorithms (excluding the ($|S|, d, d$) setting) are minimax-optimal with respect to $\alpha$.

% in which the learner interacts with $M$ source MDPs to learn a sufficient latent representation of the state, action, or both to improve the regret bound in the target MDP. In each Tucker rank setting, we introduce the transfer-ability coefficient $\alpha$ that precisely measures the difficulty of transferring a latent representation between the source and target problems.We present algorithms in each setting that combine LR-EVI (



% ; we construct information theoretic lower bounds that show a dependence on $\alpha$ in the source problem is necessary to benefit from transfer learning. We then propose algorithms that combine 


% and prove information theoretic lower bounds. 

% In setting, our algorithm combines LR-EVI, i.e., empirical dynamic programming with matrix estimation subroutine, in the source problem with a modification of LSVI-UCB, a common linear MDP algorithm \cite{Jin2020ProvablyER}, in the target problem.  



% to remove the dependence on $|S|, |A|, $ or both in the regret bound in the target MDP. 



% Furthermore, we introduce the transfer-ability coefficient that quantifies the difficulty in performing transfer learning on a specific problem. We then prove lower bounds that show our algorithms are optimal with   to the transfer-ability coefficient. 

==> content/algorithm.tex <==
\section{Algorithm}
In the source phase, our algorithm can use any algorithm that learns $\eps$-optimal $Q$ functions on each source MDP. As the error bound on the estimated feature representation depends on the incoherence of $Q^*_{h, m}$, we use LR-EVI, which combines empirical value iteration with low rank matrix estimation \cite{sam2023overcoming}.  After obtaining estimates $\bar{Q}_{m, h}$ of $Q^*_{m, h}$, our algorithm computes the singular value decompositions (SVDs) of each $\bar{Q}_{m, h}$ to construct the latent feature representation $\Tilde{F}$. Then, in the target phase, our algorithm deploys a modification of LSVI-UCB \cite{Jin2020ProvablyER} adapted to our Tucker rank setting called LSVI-UCB-(S, d, A) using the estimated feature representation $\Tilde{F}$.  For ease of notation, we define $T_{k, h}^a = \{k' \in [k] | a_h^k = a \} $, which is the set of episodes before $k$, in which action $a$ was chosen at time step $h$.
% \\\\
% \textbf{Hyperparameters:} $\{N_h\}_{h \in [H]}$, $\lambda, \beta_{k, h}^a $
% \\\\
% \textbf{Source Phase:}
% \begin{enumerate}
%     \item For each $m \in [M]$ do
% \begin{itemize}
%     \item Run LR-EVI($\{N_h\}_{h \in [H]})$ on source MDP $m$ to obtain $\bar{Q}_{m, h}$
%     \item Compute the singular value decomposition of $\bar{Q}_{m, h} = \hat{F}_{m, h} \hat{\Sigma}_{m, h} \hat{G}_{m,h}^\top$ .
% \end{itemize}
% \item Compute the feature mapping $\Tilde{F} = \{\Tilde{F}_h \}_{h \in [H]}$ with
% \[
% \Tilde{F}_h = \left \{ \sqrt{\frac{|S|}{d\mu}}\hat{F}_{m, h}(:, i)| i \in [d], m \in [M] \right\}.
% \]
% \end{enumerate}
% \textbf{Target Phase: LSVI-UCB-(S, d, A)}
% \\
% For each $k  = 1, 2, \ldots, K$ do
% \begin{itemize}
%     \item Receive initial state $s_1^k$.
%     \item For step $h = H, \ldots, 1,$ do 
%     \begin{enumerate}
%         \item For $a \in A,$ do 
%         \begin{enumerate}
%             \item Set $\Lambda_h^a \xleftarrow{} \sum_{t \in T_{k-1, h}^a} \Tilde{F}_h(s_h^t)\Tilde{F}_h(s_h^t)^\top+ \lambda \textbf{I}$
%             \item Set $w_h^a \xleftarrow{} (\Lambda_h^a)^{-1} \sum_{t \in T_{k-1, h}^a} \Tilde{F}_h(s_h^t)$ $\Big[r_h(s_h^t, a)+ \max_{a' \in A} Q_{h+1}(s_{h+1}^t, a') \Big]$
%         \end{enumerate}
%         \item For all $(s, a) \in S \times A$, set 
%         \begin{align*}
%          Q_h(s, a) &\xleftarrow[]{} \min\Big(H, \langle w_h^a, \Tilde{F}_h(s)\rangle + \beta_{k, h}^a \sqrt{ \Tilde{F}_h(s)^\top (\Lambda_h^a)^{-1} \Tilde{F}_h(s)}\Big)   
%         \end{align*}
%     \end{enumerate}
%     \item For step $h = 1, \ldots, H,$ do 
%     \begin{itemize}
%         \item Take action $a_h^k \xleftarrow[]{} \max_{a \in A} Q_h(s_h^k, a), $ and observe $s_{h+1}^k$    \end{itemize}
% \end{itemize}


\begin{algorithm}
\caption{Source Phase}\label{alg:src}
\begin{algorithmic}[1]
\Require $\{N_h\}_{h \in [H]}$
\For{ $m \in [M]$}
\State Run LR-EVI($\{N_h\}_{h \in [H]})$ on source MDP $m$ to obtain $\bar{Q}_{m, h}$.
\State Compute the singular value decomposition of $\bar{Q}_{m, h} = \hat{F}_{m, h} \hat{\Sigma}_{m, h} \hat{G}_{m,h}^\top$ .
\EndFor
\State Compute feature mapping $\Tilde{F} = \{\Tilde{F}_h \}_{h \in [H]}$ with
$
\Tilde{F}_h  = \left \{ \sqrt{\frac{|S|}{d\mu}}\hat{F}_{m, h}(:, i)|i \in [d],  m \in [M] \right\}.$
\end{algorithmic}
\end{algorithm}



\begin{algorithm}
\caption{Target Phase: LSVI-UCB-(S, d, A)}\label{alg:target}
\begin{algorithmic}[1]
\Require $\lambda, \beta_{k, h}^a, \Tilde{F} $
\For{ $k \in [K]$}
\State Receive initial state $s_1^k$.
\For {$h = H, \ldots, 1$}
\For {$a \in A$}
\State Set $\Lambda_h^a \xleftarrow{} \sum_{t \in T_{k-1, h}^a} \Tilde{F}_h(s_h^t)\Tilde{F}_h(s_h^t)^\top+ \lambda \textbf{I}$.
\State Set $w_h^a \xleftarrow{} (\Lambda_h^a)^{-1} \sum_{t \in T_{k-1, h}^a} \Tilde{F}_h(s_h^t)$ $\Big[r_h(s_h^t, a)+ \max_{a' \in A} Q_{h+1}(s_{h+1}^t, a') \Big]$.
\EndFor
\State Set $Q_h(\cdot, \cdot) \xleftarrow[]{} \min\Big(H, \langle w_h^\cdot, \Tilde{F}_h(\cdot)\rangle + \beta_{k, h}^\cdot \sqrt{ \Tilde{F}_h(\cdot)^\top (\Lambda_h^\cdot)^{-1} \Tilde{F}_h(\cdot)}\Big)  $.
\EndFor
\For{$h \in [H]$}
\State Take action $a_h^k \xleftarrow[]{} \max_{a \in A} Q_h(s_h^k, a), $ and observe $s_{h+1}^k$.
\EndFor
\EndFor
\end{algorithmic}
\end{algorithm}





LSVI-UCB-(S, d, A) uses the same mechanisms as LSVI-UCB, but we compute coefficients and gram matrices for each action. In step 5, Algorithm \ref{alg:target} computes the Gram matrix $\Lambda_h^a$ of the latent state representations whenever action $a$ was chosen in previous episodes. Step 6 updates $w_h^a$ with the solution to the regularized least squares problem, 
\begin{align*}
w_h^a &\xleftarrow[]{} \arg\min_{w \in \R^d} \sum_{t \in T_{k, h}^a} (r_h(s_h^t, a) + \max_{a' \in A} Q_{h+1}(s_{h+1}^k, a') - w^\top \Tilde{F}_h(s_h^t))^2 +  \lambda \|w\|_2^2,
\end{align*}
using the reward whenever action $a$ was chosen. Step 7 estimates the $Q$ function using the linear structure and adds the exploration bonus $\beta_{k, h}^a \sqrt{ \Tilde{F}_h(s)^\top (\Lambda_h^a)^{-1} \Tilde{F}_h(s)}$ to ensure the estimate is optimistic, which is common in linear MDP algorithms \cite{Jin2020ProvablyER, lin_band}. When constructing $\Tilde{F}$, multiplying the latent factors by $ \sqrt{|S|/(d\mu)}$ ensures that the feature mapping and coefficients are on the same scale, which is crucial in adapting the mechanisms of LSVI-UCB to our Tucker rank setting. 

While one may wonder why our modification of LSVI-UCB is necessary, Algorithm \ref{alg:src} improves the regret bound by a factor $\sqrt{|A|}$ compared to using any linear MDP algorithm. Reducing our setting to a linear MDP results in using a feature mapping with dimension $d|A|$. The lower bound from \cite{zhou2021nearly} states that the regret is lower bounded by $\Omega(\sqrt{d^2H^2T})$. Thus, using any linear MDP algorithm results in a target regret bound of at least $\Omega(\sqrt{d^2|A|^2H^2T})$. However, our algorithm shaves off a factor of $\sqrt{|A|}$ as our algorithm computes $|A|$ copies of $d \times d$ dimensional gram matrices in contrast to the $d^2|A|^2$ dimensional gram matrices used in linear MDP algorithms.
% This modification is essential to improving the regret bound in the target problem by avoiding using a linear MDP algorithm with rank $dA$, which leads to a regret bound scaling with $|A|$ instead of $\sqrt{|A|}$. The algorithms for other Tucker rank settings are essentially the same as they only differ in the construction of the latent representation and modification of LSVI-UCB. See the respective appendix for each algorithm in the different Tucker rank settings.



==> content/conclusion.tex <==
\section{Conclusion}
In this work, we study transfer RL, in which the source MDPs and target MDP have transition kernels with Tucker rank $(|S|, d, |A|), (|S|, |S|, d), (d, |S|, |A|)$ and $(|S|, d, d)$. As \cite{agarwal2023provable} studied transfer RL in the $(d, |S|, |A|)$ Tucker rank setting, our study completes the analysis of transfer RL assuming that one mode of the transition kernel is low rank. Furthermore, we propose the transfer-ability coefficient that quantifies the similarity in the latent representation between the source MDPs and target MDP and show that $\alpha$ determines the difficulty of transferring knowledge with information theoretic lower bounds. We propose computationally simple algorithms that admit regret bounds that are independent of $|S|, |A|$, or $|S||A|$ depending on the Tucker rank setting given enough samples from the source MDPs. Furthermore, these regret bounds match the bounds of algorithms that are given the true latent low-rank representation. However, our dependence on the rank and horizon is not optimal and can be improved with advanced linear MDP algorithm techniques adapted to our setting, which is an interesting open problem. Furthermore, proving theoretical guarantees of other forms of transfer learning in RL is worthwhile and an interesting future direction.

==> content/content.tex <==
\input{intro}

\input{lit_rev}

\input{preliminaries}
\input{transfer}


\input{algorithm}

\input{theory}

\input{conclusion}






==> content/intro.tex <==
\section{Introduction}
Recently, reinforcement learning (RL) algorithms have exhibited great success on a variety of problems, e.g., video games \cite{shao2019survey}, robotics \cite{rl_robotics}, etc. RL methods can be employed in any context requiring a series of decisions over time, as long as the problem can be modeled as a Markov decision process (MDP) with state space $S$, action space $A$, and horizon $H$. While RL has worked well in practice, its practical application is constrained due to the large amounts of data and computational resources required to train models that outperform heuristic approaches. This limitation arises due to the inefficient scaling of RL algorithms with respect to the size of the state and action spaces. In an online setting where rewards are incurred during the process of learning, we may want to minimize the regret, or the difference between the reward of an optimal policy and the reward collected by the learner. In the finite-horizon online episodic MDP setting with $K$ episodes, any algorithm must incur regret of at least $\Tilde{\Omega}(\sqrt{|S||A|H^3 K})$ \cite{qproveEff}. This regret bound is often too large in practice as many problems modeled as MDPs have large state and action spaces. For example, in the Atari games \cite{mnih2013playing}, the state space is the set of all images as a vector of pixel values. 

One way to remove the dependence on the state or action space in RL algorithms is to leverage existing data or models from similar problems through transfer learning. In the transfer learning setting for MDPs, the learner can interact with or query from multiple source MDPs, which the learner can utilize at low-cost to improve their performance in the target MDP \cite{transfer_learning}. The efficacy of the transfer learning approach depends both on the similarity between the source and the target MDPs, and how information is utilized when transferring knowledge between the source and target.

In this work, we consider a setting when the source and target MDPs exhibit latent low rank structure, and the transfer RL task is to use the source MDPs to learn the latent low rank representation of the state, action, or state-action pair, and subsequently use the representation to improve learning on the target MDP.  If the learned representations were perfect, then one could remove all dependence on the state space or action space in the learning task on the target MDP. This approach relies on a critical assumption that the transition kernels of the \cyedit{source and target} MDPs have low Tucker rank when viewed as a $|S|$-by-$|S|$-by-$|A|$ tensor. 

The work \cite{agarwal2023provable} studied this problem in the Low Rank MDP setting, \cyedit{when the transition kernel is low rank along the first mode, i.e. Tucker rank $(d,|S|,|A|)$}.
We consider the \cyedit{complementary} settings in which the transition kernel has low Tucker rank along the second mode or third mode, i.e., Tucker rank $(|S|, d, |A|)$ or $(|S|, |S|, d)$, respectively, as introduced in \cite{sam2023overcoming}, in addition to the $(d, |S|, |A|)$ setting. We also study the $(|S|, d, d)$ Tucker rank setting as we can further exploit the low rank structure to improve performance in the target problem. \cyedit{The different modes are not interchangeable algorithmically as there is a directionality due to the time of the transition between the current and future state. Additionally, the algorithm in \cite{agarwal2023provable} is not computationally tractable as it utilizes an optimization oracle which may not be practical, and they assume that the latent representations are within a known finite function class. Our work proposes a computationally efficient algorithm that can handle latent low rank structure on the transition kernel along any of the three different modes.}
%While the sample complexity in the source MDPs has a necessary dependence on $|S|$ and $|A|$, the transfer learning approach removes dependence on $|S|$ and $|A|$ in the performance on the target MDP.

As the success of a transfer learning approach depends on the similarity between the source and target problems, we introduce the transfer-ability coefficient $\alpha$ \tscomment{name in progress} that quantifies the similarity between the source and target problems under our low rank assumptions, which is similar to the task-relatedness in \cite{agarwal2023provable} and unique to the transfer reinforcement learning setting. 

\paragraph{Our Contributions:} We propose new computationally efficient transfer RL algorithms that admit the desired efficient regret bounds under our low Tucker rank assumptions ($(|S|, d, |A|)$, $(|S|, |S|, d), (d, |S|, |A|)$, and $(|S|, d, d)$). With enough samples from the source MDPs, we remove the dependence on $|S|, |A|, $ or $|S||A|$ in the regret bound on the target MDP. In addition, we introduce the transfer-ability coefficient that measures the ease of transferring a latent representation between the source MDPs and target MDP. We also show that our algorithms are optimal with respect to $\alpha$ with information theoretic lower bounds under our Tucker rank settings. In the $(d, |S|, |A|)$ Tucker rank setting, our information theoretic lower bound shows that our dependence of $\alpha^2$ is optimal while \cite{agarwal2023provable} is sub-optimal with a dependence on $\alpha^5$.

\yccomment{Talk about simulator-to-simulator setting somewhere in the main text?}

==> content/lit_rev.tex <==
\section{Related Work}
\paragraph{Transfer RL:}
The work most closely related to ours is \cite{agarwal2023provable}, which performs reward-free exploration in the source problem to learn a sufficient representation to use in the target problem in the $(d, |S|, |A|)$ Tucker rank setting. They propose a task relatedness coefficient, which captures the existing representational transfer RL settings \cite{cheng2022provable} and is similar to our transferabillity coefficient but differs due to the different low rank assumptions. \cite{cheng2022provable, lu2021power} require stronger assumptions on the given function class to enable transfer learning. Their algorithm admits a source sample complexity bound of $\Tilde{O}(A^4\alpha^3d^5H^7K^2T\log(|\Phi|))$ with a target regret bound of $\Tilde{O}(\sqrt{d^3 \alpha^2H^4 T})$.
Similar to transfer RL, reward free RL studies the problem of giving the learner access to only the transition kernel in the first phase, and in the second phase the learner must output a good policy when given multiple reward functions \cite{Jin2020RewardFreeEF, zhang2020taskagnostic, cheng2023improved}. While reward free RL is similar to our setting, enabling the dynamics to differ between the source and target phase greatly increases the difficulty and changes the objective in the source problem, i.e., learning a good latent representation instead of collecting trajectories that sufficiently explore the state space. 

\paragraph{RL in the $(d, |S|, |A|)$ Tucker rank Setting:}
There exists an extensive body of literature on MDPs in the $(d, |S|, |A|)$ Tucker rank setting. Linear MDPs assume that the dynamics are linear with respect to a known feature mapping $\phi$. These works use the feature mapping $\phi$ to remove all dependence on the size of the state and action spaces and replace it with the rank $d$ of the latent space\cite{Jin2020ProvablyER, yang2019sampleoptimal, pmlr-v119-yang20h, wang2021sampleefficient}. \cite{he2023nearly} proposes an algorithm that admits a regret bound of $\Tilde{O}(\sqrt{d^2H^2T})$, which matches the known lower bounds. Our algorithm in the target phase modifies existing linear MDP algorithms to take advantage of the knowledge learned in the source phase. Low Rank MDPs impose the same low-rank structure as linear MDPs but assume that $\phi$ is unknown. To avoid dependence on the size of the state space, many works in this setting construct algorithms that utilize a computationally inefficient oracle to admit sample complexity or regret bounds that scale with the size of the action space and the log of the size of the function class the true low rank representation \cite{flambe, uehara2021representation, moffle, briee}. In contrast, \cite{pro_rl} incurs sample complexity on $|S||A|$ instead of the size of the function class to learn near-optimal policies using matrix estimation in reward free low-rank MDPs. 

\paragraph{RL in the $(|S|, d, |A|)$ or $(|S|, |S|, d)$ Tucker Rank Setting: }
\cite{sam2023overcoming} introduces the RL setting in which the transition kernel has Tucker rank $(|S|, d, |A|)$ or $(|S|, |S|, d)$. With access to a generative model, their algorithms learn near-optimal polices with sample complexities that scale with $|S|+|A|$ instead of $|S||A|$, which is the lower bound for tabular reinforcement learning \cite{azarLowerBound}. \cite{xi2023matrix} consider the same low Tucker rank assumption on the dynamics but in the offline RL setting. \cite{Yang2020Harnessing, lrVfa, mlrvfa} empirically show the benefits of combining matrix/tensor estimation with RL algorithms on common stochastic control tasks. \cite{jedra2024lowrank} consider the low-rank bandits setting and use a similar algorithm to ours by estimating the singular subspaces of the reward matrix to improve the regret bound's dependence on the dimension of the problem. 


==> content/preliminaries.tex <==
\section{Preliminaries}
We consider the transfer reinforcement learning setting introduced by \cite{agarwal2023provable}, in which
the learner interacts with $M$ finite horizon source MDPs and one finite horizon episodic target MDP. All MDPs share the same discrete state space $S$, discrete action space $A$, and finite horizon $H\in \Z_+$. \tscomment{We don't need to share the same state or action space depending on which Tucker rank setting we are in. Note that depending on the Tucker rank of the transition kernel, we only require the source and target MDPs share only one of the spaces.} $r = \{r_h\}_{h \in [H]}$ is the deterministic unknown reward function of the target MDP where $r_h: S \times A \to [0, 1]$. $r_m = \{r_{m, h}\}_{h\in [H]}$ for $m \in [M]$ is the deterministic unknown reward function for source MDP $m$ where $r_{m, h}: S \times A \to [0, 1]$ \footnote{Our results can easily be extended to stochastic reward functions.}. $P = \{P_h\}$ is the transition kernel for the target MDP where $P_h(s'|s, a)$ is the probability of transitioning to state $s'$ from state-action pair $(s, a)$ at time step $h$. Similarly, $P_m$ for $m \in [M]$ is defined in the same way as $P$ and is the transition kernel for source MDP $m$. An agent's policy has the form $\pi = \{\pi_h\}_{h\in [H]}, \pi_h: S\to \Delta(A)$, where $\pi_h(a|s)$ is the probability that the agent chooses action $a$ at state $s$ and time step $h$. The value function and action-value ($Q$) function of a policy $\pi$ are the expected reward of following $\pi$ given a starting state and starting action, respectively, beginning at time step $h$. We define these as 
\[
V^\pi_h(s) \coloneqq \E\left[\sum_{t = h}^H r_t(s_t, \pi_t(s_t))| s_h = s \right], \quad Q^\pi_h(s, a) \coloneqq \E\left[\sum_{t = h}^H r_t(s_t, a_t)| s_h = s, a_h = a \right]
\]
where $a_t \sim \pi_t(s_t), s_{t+1} \sim P_t(\cdot|s_t, a_t)$. The optimal value function and action value function are $V^*_h(s) \coloneqq \sup_\pi V^\pi_h(s), Q^*_h(s, a) \coloneqq \sup_\pi Q^\pi_h(s, a)$ for all $(s, a, h) \in S \times A \times [H]$ and satisfy the Bellman equations $V^*_h(s) = \max_{a \in A}Q^*_h(s, a), Q^*_h(s, a) = r_h(s, a) + E_{s'\sim P_h(\cdot|s, a)}[V^*_{h+1}(s')]$ for all $(s, a, h) \in S \times A \times [H]$. We define an $\eps$-optimal policy $\pi$ for $\eps > 0$ as any policy that satisfies $V^*_h(s) - V^\pi_h(s) \leq \eps$ for all $s \in S, h \in [H]$. Similarly, $Q$ is $\eps$-optimal if $Q^*_h(s, a) - Q_h(s, a) < \eps$ for all $(s, a, h) \in S \times A \times [H]$. Also, we use the shorthand $P_h V (s, a) = \E_{s'\sim P_h(\cdot|s, a)}[V(s')]$. 

In the transfer RL problem, the learner first interacts with the $M$ source MDPs without access to the target MDP in the source phase. In this phase, the learner is given access to a generative model in each of the source MDPs. The generative model takes in a state-action pair $(s, a)$ and time step $h$ and outputs $r_h(s, a)$ and an independent sample from $P_h(\cdot|s, a)$ \cite{NIPS1998_99adff45}. Access to a generative model in the source phase is necessary to learn a latent low rank representation; Theorem 4.1 in \cite{agarwal2023provable} states that without access to a generative model in the source phase, one cannot learn a near-optimal policy in the target phase using the learned representation. Then, in the target phase, the learner loses access to the source MDPs and interacts only with the target MDP without access to a generative model. The performance of the learner is evaluated by not only the regret in the target MDP, i.e., $Regret(T) = \sum_{k \in [K]} V^*_1(s) - V^{\pi^k}_1(s)$ where $\pi^k$ is the learner's policy in episode $k$ but also the number of samples taken in the source phase. 

\subsection{Low Tucker Rank MDPs}
For the reader's convenience, we first present the definition of the Tucker rank of a tensor.
\begin{definition}[Tucker Rank~\cite{tucker}] 
\label{def:tr}
A tensor $M \in \R^{n_1 \times n_2 \times n_3}$ has Tucker rank $(d_1, d_2, d_3)$ if $(d_1, d_2, d_3)$ is the smallest such that there exists a core tensor $X \in \R^{d_1 \times d_2 \times d_3}$ and orthonormal latent factors $G_i \in \R^{n_i}$ for $i \in [3]$ such that 
\begin{align*}
&M(a, b, c) = \textstyle\sum_{i \in [d_1], j \in [d_2], k \in [d_3]} X(i, j, k) G_1(a, i)G_2(b, j) G_3(c, k).
\end{align*}
\end{definition}

In standard MDPs, the transition kernel has Tucker rank $(|S|, |S|, |A|)$ as there is no low rank structure imposed on the tensor. In this work, we analyze the benefits of assuming that the transition kernel is low rank along each mode/dimension of the transition kernel, which corresponds to the $(|S|, d, |A|), (|S|, |S|, d),$ and $(d, |S|, |A|)$ Tucker rank settings. Additionally, we analyze the $(|S|, d, d)$ Tucker rank setting as we can further exploit the low rank structure to improve the regret bound in the target phase when compared to the $(|S|, d, |A|)$ and $(|S|, |S|, d)$ Tucker rank settings. In each setting, we present an algorithm with theoretical guarantees that admit efficient target phase regret bounds that remove the dependence on $|S|, |A|,$ or $|S||A|$. On the other hand, utilizing the low rank structure imposed in the $(d, |S|, d)$ or $(d, d, |A|)$ Tucker rank settings requires novel mechanisms. In these settings, one learns low rank representations of the state and next state $\phi(s, s')$ or action and next state $\phi(a, s')$, which differs significantly from our setting and the related literature. \yccomment{I don't quite understand this sentence.}

While the sample complexity and regret bound of each algorithms differ in each setting, one should choose which algorithm to use based on the low rank structure inherent in their
problem. For example, in the $(|S|, d, |A|)$ Tucker rank setting, one assumes that the state one transitions from has a low rank representation. Similarly, in the $(|S|, |S|, d)$ Tucker rank setting, each action can be mapped to a lower dimensional space. The $(|S|, d, d)$ Tucker rank setting combines the two previous assumptions and asserts that current states and actions have separate low dimensional representations. In contrast, in low rank MDPs (the $(d, |S|, |A|)$ Tucker rank setting), one assumes that each state-action pair has a joint low rank representation. \yccomment{For $(d,S,A)$, we can also say the next state has a low-dimensional representation?}

We first define the incoherence $\mu$ of a matrix as it is used in the regularity conditions of our Tucker rank assumption. 
\begin{definition}\label{def:inco}
    Let $X \in \R^{m \times n}$ have rank $d$ with singular value decomposition $X = U\Sigma V^\top$ with $U \in \R^{m \times d}, V\in \R^{n \times d}$. Then, $X$ is $\mu$-incoherent if  for all $i \in [m], j \in [n]$,
    \[
    \|U(i, :)\|_2 \leq \sqrt{d\mu/m}, \quad \|V(j, :)\|_2 \leq \sqrt{d\mu/n}.
    \]
    
\end{definition}
A small incoherence parameter $\mu$ guarantees that the signal in $U$ and $V$ is sufficiently spread out among the rows in those matrices. 

For sake of brevity, we will only present our assumption and algorithm for the $(|S|, d, |A|)$ Tucker rank setting in the main body of this work and defer the other settings to the appendix. 
Introduced in \cite{sam2023overcoming}, we assume that reward functions are low rank and the transition kernels have low Tucker rank in each of the source and target MDPs. 

\begin{assumption}\label{asm:tr}
In each of the $M$ source MDPs and the target MDP, the reward functions have rank $d$, and the transition kernels have Tucker rank $(|S|, d, |A|)$. Thus, there exists $|S| \times d \times |A|$ tensors $U_{m, h}, U_h$, $|S| \times d$ orthonormal matrices $F_{m, h}, F_h$ that are $\mu$-incoherent, and $|A| \times d$ matrices $W_{m, h}, W_{ h}$ such that 
\begin{align*}
P_{m, h}(s'|s, a) &= \textstyle\sum_{i \in [d]} F_{m, h}(s, i)U_{m, h}(s', a, i) , \quad 
r_{m, h}(s, a) = \textstyle\sum_{i \in [d]} F_{m, h}(s, i) W_{m, h}(a, i)
\end{align*}
and 
\begin{align*}
P_{h}(s'|s, a) &= \textstyle\sum_{i \in [d]} F_h(s, i)U_h(s', a, i) , \quad
r_{ h}(s, a) = \textstyle\sum_{i \in [d]} F_h(s, i) W_{ h}(a, i)
\end{align*}
where $\|\sum_{s' \in S} g(s') U_{m, h}(s', :, a)\|_2$, $ \|\sum_{s' \in S}g(s') U_{ h}(s', :, a)\|_2, \|W_{h}(a)\|_2, \|W_{m, h}(a)\|_2 \leq \sqrt{|S|/(d\mu)} $ for all $s \in S$, $a \in A$, $h\in[H]$, and $m\in [M]$ for any function $g:S \to [0, 1]$. 
\end{assumption}
The main benefit of Assumption \ref{asm:tr} is that for any value function $V$, the Bellman update of any value function, $Q_h = r_h + P_hV$, is a low rank matrix due to Proposition 4 \cite{sam2023overcoming}. Figure \ref{fig:tr} visualizes the low rank structure Assumption \ref{asm:tr} imposes on the transition kernel. 
% \begin{figure}[h]
%     \centering
%     \includegraphics[width = 0.4\textwidth]{img/Tucker_rank_sda.PNG}
%     \caption{Transition kernel with Tucker rank  $(|S|, d, |A|)$}
%     \label{fig:tr}
% \end{figure}
\begin{figure}
\centering
\begin{minipage}[t]{.45\textwidth}
  \centering
\includegraphics[width =\textwidth]{img/Tucker_rank_sda.PNG}
\caption{Transition kernel with Tucker rank  $(|S|, d, |A|)$}
\label{fig:tr}
\end{minipage}%
\quad
\begin{minipage}[t]{.45\textwidth}
  \centering
\resizebox{\textwidth}{!}{%
\begin{circuitikz}
\tikzstyle{every node}=[font=\small]
\draw [](7.25,8.5) to[short] (9,8.5);
\draw [](7.5,10) to[short] (7.5,8.25);
\draw [->, >=Stealth] (7.5,8.5) -- (7.5,10);
\node [font=\tiny] at (7.5,10.25) {$F_T = [0, 1]$};
\draw [->, >=Stealth] (7.5,8.5) -- (9,8.5);
\node [font=\tiny] at (9.75,8.5) {$F_1 = [1, 0]$};
\draw [->, >=Stealth] (7.5,8.5) -- (9,8.75);
\node [font=\tiny] at (10.45,8.875) {$F_2 = [\sqrt{1 - 1/\alpha^2}, 1/\alpha]$};
\end{circuitikz}
}%
\caption{ A difficult representational transfer example where one estimates $F_T$ with $F_1$ and $F_2$}
\label{fig:alpha}
\end{minipage}
\end{figure}
While Assumption \ref{asm:tr} states that the source MDPs and target MDPs have latent low rank structure, the assumption does not guarantee that low rank representations are similar. Thus, to allow for transfer learning to occur by transferring a latent low rank representation between the source and target MDPs, we assume the space spanned by the target latent factors is a subset of the space spanned by the latent factors from all source MDPs.
\begin{assumption}\label{asm:transfer}
Suppose Assumption \ref{asm:tr} holds.For latent factors $F_h$ from the target MDP and $F_{m, h}$ for the source MDPs, let $F_h = \{F_h, F_{h, m}\}_{m\in [M]}$. Then, there exists a non-empty set $\B(F_h)$ such that the elements in $\B(F_h)$ are $B_h \in \R^{d, d, M}$ such that for all $i \in [d], s \in S, h \in [H]$,
\[
F_h(s, i) = \textstyle\sum_{j \in [d], m \in [M]} B_h(i, j, m) F_{m, h}(s, j).
\]

\end{assumption}

Assumption \ref{asm:transfer} asserts that the space spanned by the target latent factors $\{F_h(:, i)\}_{i \in [d]}$ is a subset of the space spanned by source latent factors $\{F_{m, h}(:, i)\}_{i \in [d], m \in [M]}$. Thus, by learning $F_{m, h}$, we can construct a latent feature representation in the source problem that approximates $F_h$ \textbf{without interacting} with the target MDP, which is essential to transfer learning. To learn each latent factor, one needs to obtain a good estimate of a suitably large rank $d$ matrix. Therefore, we assume that the optimal $Q$ functions in each source MDP are full rank with the largest entry lower bounded by a constant.

\begin{assumption}\label{asm:full_rank}
    For each $m \in [M], h \in [H]$, the optimal $Q$ function satisfies $rank(Q^*_{m, h}) = d$ and $\|Q^*_{m, h}\|_\infty \geq C$ for some $C \in \R^{+}$.
\end{assumption}

The above assumption determines our goal in the source phase, i.e., learning near-optimal $Q$ functions. Without the above assumption (the rank of $Q^*$ is strictly less than $d$), then one cannot learn every latent factor $F_{m, h}(:, i)$ and using the approximate feature mapping would result in regret linear in $T$. Similarly,  $\|Q^*\|_\infty \geq C$ ensures that some entries of $Q^*$ are sufficiently large and prevents the noise from dominating the low rank signal that one learns in the source phase.
% hence, one may learn the low rank representation from the noise instead of $Q^*$ and render transfer learning useless. Assuming that the largest entry of $Q^*$ is lower boudned by a constant eliminates this issue. 

% Furthermore, we let $D = \min_{h \in [H], m \in [M]} \|Q^*_{h, m}\|_\infty$ as the magnitude of the $Q^*_{m, h}$ also determines the difficulty in estimating those matrices.


==> content/theory.tex <==
\section{Theoretical Results}
In this section, we prove our main theoretical results that show with enough samples in the source problem, our algorithms admit regret bounds that are independent of $|S|, |A|,$ or both $|S|$ and $|A|$ in the target problem. We first state our main result in the $(|S|, d, |A|)$ Tucker rank setting.

\begin{thm}\label{thm:tl_sda}
Suppose Assumptions \ref{asm:tr}, \ref{asm:transfer}, and \ref{asm:full_rank} hold, and set $\delta \in (0, 1)$. Furthermore, assume that all the state latent factors are $\mu$-incoherent, and for any $\eps > 0$, that $Q_{m, h} = r_{m, h} + P_{m, h} V_{m, h+1}$ has rank $d$ and is $\mu$-incoherent with condition number $\kappa$ for all $\eps$-optimal value functions $V_{h+1}$. Also, let $\lambda = 1,  \beta_{k, h}^a = C(Hd\sqrt{\iota} + \xi\sqrt{d |T^a_{k, h}|}H)$ for some absolute constant $C> 0$. Then, for $T \geq  \frac{|A|}{ \alpha^2}$, using at most $\Tilde{O} \left( d^4 \mu^4\kappa^4(|S|/|A|+1)M^2  H^4\alpha^2  T \right) $ samples in the source problems, our algorithm has regret at most $\Tilde{O}\left( \sqrt{(dMH)^3 |A|T}\right)$ with probability at least $1 - \delta$.
\end{thm}
Theorem \ref{thm:tl_sda} states that using transfer learning greatly improves the performance on the target problem by removing the regret bound's dependence on the state space. Thus, with enough samples from the source MDPs one can recover a regret bound in the target problem that matches the best regret bound for any algorithm in the $(|S|, d, |A|)$ Tucker rank setting with \textbf{known} latent feature representation $F$ concerning $|A|$ and $T$. 

\yccomment{Need to better organize these quantitative discussions; some may be moved to Section \ref{sec:discussion-optimality}.}
While the source sample complexity may seem independent of $|A|$, we require the horizon in the target phase to be large enough $(T\alpha^2 \geq |A|)$ so that one observes $\Omega(|S|+|A|)$ samples in the source phase. The source sample complexity's scaling with respect to $|S|, |A|,$ and $H$ are typical when learning  $\sqrt{|A|/T}$-optimal $Q$ functions in this Tucker rank setting while our dependence on $\alpha$ is optimal due to our lower bound, Theorem \ref{thm:lb_tr}. Similarly, the dependence on $\mu$ and $\kappa$ are standard for methods incorporating matrix estimation. In Appendix \ref{app:gen}, we show the benefit of transfer learning in the $(|S|, d, |A|)$ Tucker rank setting when the learning is given the generative model in both the source and target phases. 


For sake of brevity, we present our results in our other Tucker rank settings in Table \ref{tab:tr_all}\footnote{The source sample complexities in Table \ref{tab:tr_all} suppress the dependence on matrix estimation terms, i.e., the incoherence, condition number, and magnitude of the largest entry.} (see Appendices \ref{app:tr_ssd}, \ref{app:tr_dsa}, and \ref{app:tr_sdd} for the formal statements and proofs).
\begin{table}
    \centering
    \begin{tabular}{|c|c|cc|}
    \hline
        & Tucker Rank Setting & Source Sample Complexity & Target Regret Bound  \\
       \hline
       Theorem \ref{thm:tl_sda} &$(|S|, d, |A|)$ & $\Tilde{O}  \left(d^4 (|S|/|A|+1)M^2  H^4\alpha^2  T \right) $ & $\Tilde{O}\left( \sqrt{(dMH)^3 |A|T}\right)$ \\
        Theorem \ref{thm:tl_ssd} &$(|S|, |S|, d)$ & $\Tilde{O}  \left(d^4 (1+|A|/|S|)M^2  H^4\alpha^2  T \right) $ & $\Tilde{O}\left( \sqrt{(dMH)^3 |S|T}\right)$ \\
        Theorem \ref{thm:tl_dsa}  & $(d, |S|, |A|)$ & $\Tilde{O} \left(\alpha^2 d M^2 T  |S||A| \right)$& $\Tilde{O}\left( \sqrt{(dMH)^3T}\right)$  \\
        Theorem \ref{thm:tl_sdd} & $(|S|, d, d)$ & $\Tilde{O} \left( d^{10} (|S|+|A|)M^2  H^4 \alpha^4 T\right)$& $\Tilde{O}\left( \sqrt{d^6M^6 H^3T}\right)$\\
        \hline
    \end{tabular}
    \caption{Theoretical guarantees of our algorithms in our different Tucker rank settings}
    \label{tab:tr_all}
\end{table}
% If the actions in one's problem exhibit low rank structure, then one can adapt our algorithm to the $(|S|, |S|, d)$ Tucker rank setting, which results in the following theorem (See Appendix \ref{app:tr_sda} for the setting, algorithm, and proof).
Similarly, the source sample complexity in the $(|S|, |S|, d)$ Tucker rank setting is minimally $\Omega(|S| + |A|)$ as we require $T\alpha^2$ to be sufficiently large. In each of our Tucker rank settings, our algorithms use transfer learning to remove the dependence on $|S|, |A|, $ or $|S||A|$ in the target regret bound, which matches the dependence on $|S|$ and $|A|$ of the best regret bounds of algorithms with \textbf{known} latent representation.

In the $(|S|, |S|, d)$ and $(d, |S|, |A|)$ Tucker rank settings, our dependence on $d, H, M,$ and $T$ in the source sample complexity are reasonable while our dependence on $\alpha$ is optimal due to our lower bounds. In the $(|S|, d, d)$ Tucker rank setting, our $\alpha^4$ dependence is likely optimal when one wants to eliminate the dependence on $|S|$ and $|A|$ in the target problem; one must multiply both sets of singular vectors together to create a feature mapping $\phi:|S||A| \to d^2M^2$, which causes the $\alpha^4$ dependence in our upper bound. However, if $\alpha^4$ is too large, one can use the algorithms from the $(|S|, d, |A|)$ or $(|S|, |S|, d)$ Tucker rank settings to improve performance on the target problem. We believe proving the $\alpha^4$ lower bound is an interesting open question. Additionally, the dependence on $d$ and $M$ in this setting is worse as our low rank latent representation of each state-action pair lies in a $d^2M^2$ dimensional space in contrast to a space with dimension $dM$.

In comparison to Theorem 3.1 \cite{agarwal2023provable}, our result, Theorem \ref{thm:tl_dsa}, has similar dependence on $|A|, d, H,$ and $T$ while our dependence on $\alpha$ is optimal compared to their $\alpha^5$ dependence \footnote{Since $\bar{\alpha} \geq \alpha $,  moving $\bar{\alpha}$ into the source sample complexity yields a sample complexity that scales with $\alpha^5$.}. While our dependence on $M$ in the regret bound is worse, this is due to our transfer learning setting being more general; we only require that the space spanned by the target features be a subset of the space spanned by the source features instead of having the target features being a linear combination of the source features. Furthermore, our source sample complexity scales with the size of the state space instead of scaling logarithmically in the size of the given function class.






% a modification of our algorithm removes the dependence on the size of the action space in the target regret bound. Furthermore, the target regret bound matches the regret bounds of algorithms in the $(|S|, |S|, d)$ Tucker rank setting with \textbf{known} latent representation. The scalings with respect to $|S|, |A|, T$ in the source sample complexity are reasonable while the dependence on $\alpha$ is optimal. 

% If both states and actions have separate low rank representations in one's application, modifying our algorithm to the $(|S|, d, d)$ Tucker rank setting results in a target regret bound that removes the dependence on both $|S|$ and $|A|$ (see Appendix \ref{app:tr_sdd} for the setting, algorithm, and proof).



% Theorem \ref{thm:tl_sdd} shows that the modification of our algorithm in the $(|S|, d, d)$ admits a regret bound in the target phase that matches the regret of linear MDP algorithms with respect to $T, |S|,$ and $|A|$. In contrast to the previous two Tucker rank settings, one needs to estimate both sets of singular vectors and multiply them together to construct a latent low rank representation with dimension $d^2M^2$, which increases the scalings with respect to $d, \mu,$ and $\kappa$. Thus, we think our $\alpha^4$ dependence is likely optimal when one wants to remove the dependence on $|S|$ and $|A|$ in the target problem; however, we leave proving this lower bound as an open problem. If $\alpha^4$ is too large, one can use the algorithms from the $(|S|, d, |A|)$ or $(|S|, |S|, d)$ Tucker rank settings to improve performance on the target problem. 

% If one expects each state-action pair to have a joint low rank representation (low rank MDPs), then a modification to our algorithm yields the following result (see Appendix for the setting, algorithm, and proof.)


% Like the previous theorems, the benefit of the transfer learning approach in the $(d, |S|, |A|)$ Tucker rank setting is removing the dependence on both $|S|$ and $|A|$ in the target regret bound. In comparison to Theorem 3.1 \cite{agarwal2023provable}, our result has similar dependence on $|A|, d, H,$ and $T$ while our dependence on $\alpha$ is optimal compared to their $\alpha^5$ dependence \footnote{Since $\bar{\alpha} \geq \alpha $,  moving $\bar{\alpha}$ into the source sample complexity yields a sample complexity that scales with $\alpha^5$.}. While our dependence on $M$ in the regret bound is worse, this is due to our transfer learning setting being more general; we only require that the space spanned by the target features be a subset of the space spanned by the source features instead of having the target features being a linear combination of the source features. Furthermore, our source sample complexity scales with the size of the state space instead of scaling logarithmically in the size of the given function class.

%  In contrast to our approaches in the other Tucker rank settings, one learns the latent representation in the source MDPs through the transition kernels. One potential issue arises when all entries of $P(\cdot| \cdot, a)$ are small; for example, each entry of the uniform transition kernel is $1/|S|$, which is not lower bounded by a constant. Thus, the dependence on $D = \min_{m \in [M], h \in [H], a \in A} \|P_{m, h}(\cdot | \cdot, a)\|_\infty$ is unsurprising as one needs to ensure the noise is sufficiently small to learn the latent representations from $P_{m, h}$.  

The proofs of Theorem \ref{thm:tl_sda}, \ref{thm:tl_ssd}, \ref{thm:tl_sdd}, and \ref{thm:tl_dsa} synthesize the theoretical guarantees of LR-EVI, singular vector perturbation bounds, and LSVI-UCB or our modification of LSVI-UCB. Given $N$ samples from the source MDPs, we first bound the error between the singular subspaces up to a rotation by $ \sqrt{d^3M(|S| + |A|)/N}$ (suppressing the dependence on common matrix estimation terms) to construct our feature mapping. 
Thus, with enough samples in the source MDPs,  LR-EVI returns $Q$ functions with singular vectors that can be used to construct a sufficient feature representation; the additional regret incurred from using the approximate feature representation in LSVI-UCB or Algorithm \ref{alg:target} is dominated by the original regret of using the true representation.
% Modifying LSVI-UCB results in our algorithms admitting regret bounds that are independent of $|S|$, $|A|$, or $|S||A|$.

\subsection{Discussion of Optimality}
\label{sec:discussion-optimality}

The regret bounds of our algorithms with used in the target phase are optimal with respect to $|S|,|A|,$ and $T$. Since each Tucker rank setting captures tabular MDPs, we can construct lower bounds with a reduction from the bound in \cite{qproveEff}, e.g., in the $(|S|, d, |A|)$ setting,   the regret is at least $\Tilde{\Omega}(\sqrt{d|A|H^2 T})$. However, our dependence on $d$ and $H$ are sub-optimal. 
% The extra factor of $\sqrt{H}$ is likely due to our choice of exploration bonus by adapting LSVI-UCB as we don't utilize the variance of the estimates. 
The extra factor of $\sqrt{H}$ is likely due to our use of Hoeffding's inequality instead of tracking the variance of the estimates and using Bernstein's inequality. Our dependence on $d$ is sub-optimal as LSVI-UCB is sub-optimal with respect to $d$; for linear MDPs, LSVI-UCB++ \cite{he2023nearly} admits a regret bound of $\Tilde{O}(\sqrt{d^2H^2T})$, which matches the lower bound from \cite{zhou2021nearly}. Thus, to obtain the optimal dependence on $d$ and $H$, we would need to adapt LSVI-UCB++ to our Tucker rank setting. 

% While one may wonder why our modification of LSVI-UCB is necessary, Algorithm \ref{alg:src} improves the regret bound by a factor $\sqrt{|A|}$ compared to using any linear MDP algorithm in the $(|S|, d, |A|)$ Tucker setting. Reducing our Tucker rank setting to a linear MDP results in using a feature mapping with dimension $d|A|$. The lower bound from \cite{zhou2021nearly} states that the regret is lower bounded by $\Omega(\sqrt{d^2H^2T})$. Thus, using any linear MDP algorithm results in a target regret bound of at least $\Omega(\sqrt{d^2|A|^2H^2T})$. However, our algorithm shaves off a factor of $\sqrt{|A|}$ as our algorithm computes $|A|$ copies of $d \times d$ dimensional gram matrices ($|A| \times d^2$ compared to $d^2|A|^2$ dimensional gram matrices in linear MDP algorithms).


% in the target regret bound. The main reason is that in linear MDP algorithms, computing gram matrix $\Lambda$ used in the least squares estimation step has dimension $d|A| \times d|A|$. However, in our modification of LSVI-UCB, we instead have $|A|$ copies of $d \times d$ dimensional gram matrices ($|A| \times d^2$ compared to $d^2|A|^2$).


% textbf{Move Theoretical Guarantees of the Algorithm to the Appendix}


==> content/transfer.tex <==

\section{Transfer-ability}
As the similarity between the source and target problems plays a pivotal role in the effectiveness of transfer learning, we propose the transfer-ability coefficient $\alpha$. 
% $\alpha$ quantifies the difficulty of transferring a latent representation from the source MDPs to the target MDP.

\begin{definition}[Transfer-ability Coefficient]\label{def:tc}
Given a transfer RL problem that satisfies Assumptions~\ref{asm:tr}, \ref{asm:transfer}, and \ref{asm:full_rank}, let $\mathcal{F}$ be the set of all $\R^{|S| \times d}$ orthonormal latent factor matrices with columns that span the column space of $Q^*_{m, h}$ for all $m \in [M], h \in [H]$. Then, we define $\alpha$ as 
\[
\alpha \coloneqq \min_{F \in \mathcal{F}}\min_{B \in \B(F)} \max_{i, j \in [d], m\in [M]} |B(i, j, m)|.
\]
\end{definition}
While transfer learning is possible as long as Assumption \ref{asm:transfer} holds, $\alpha$ precisely measures the challenge involved in transferring the latent representation. Figure \ref{fig:alpha} depicts an example where transfer learning is possible but very difficult, i.e., $\alpha$ is large; the estimation error of $F_1$ and $F_2$ are amplified by $\alpha$ when estimating $F_T$ using $F_1$ and $F_2$.  
\yccomment{Is 1 the smallest possible value of $\alpha$? What does it mean when $\alpha =1$?}
% \begin{figure}[h]
% \centering
% \resizebox{.4\textwidth}{!}{%
% \begin{circuitikz}
% \tikzstyle{every node}=[font=\small]
% \draw [](7.25,8.5) to[short] (10,8.5);
% \draw [](7.5,11) to[short] (7.5,8.25);
% \draw [->, >=Stealth] (7.5,8.5) -- (7.5,11);
% \node [font=\tiny] at (7.5,11.25) {$F_T$};
% \draw [->, >=Stealth] (7.5,8.5) -- (10,8.5);
% \node [font=\tiny] at (10.25,8.5) {$F_1$};
% \draw [->, >=Stealth] (7.5,8.5) -- (10,8.75);
% \node [font=\tiny] at (10.25,8.75) {$F_2$};
% \end{circuitikz}
% }%
% \caption{A transfer learning example when the source latent factors are $[1, 0], [\sqrt{1 - 1/\alpha^2}, 1/\alpha]$ and the target latent factor is $[0, 1]$.}
% \label{fig:alpha}
% \end{figure}


% To illustrate why $\alpha$ captures the difficulty of transferring knowledge between the source and target MDPs, we consider the following example with two transfer RL problems with state and action space being $\{0, 1\}$ with $H = 1$ where the learner is given one of the problems with equal probability. The first target MDP has latent factor $[0, 1]^\top$ while the second has latent factor $[1, 0]^\top$. The optimal $Q$ functions for transfer RL problems one and two are 
% \[
% Q^*_1 = \left[\begin{tabular}{cc}
%          0& 1  \\
%           0& 1  \end{tabular} \right] 
%          \text{ and } Q^*_2 = \left[\begin{tabular}{cc}
%          0 & 1  \\
%          $1/\alpha$ & $\sqrt{1 - 1/\alpha^2}$  \end{tabular} \right], 
% \]
% respectively. Even if the learner is given that the target latent factor is in $\{ [0, 1]^\top, [1, 0]^\top\}$, they need to distinguish between $Q^*_1$ and $Q^*_2$ to choose the correct target latent factor. Since $\|Q^*_1 - Q^*_2\|_\infty \leq 1/\alpha$, it is harder for the learner to distinguish between $Q^*_1$ and $Q^*_2$ as $\alpha$ increases. Thus, $\alpha$ quantifies the difficulty in transfer knowledge from the source problem to the target problem. See Appendix \ref{app:alpha_ex} for an example with large $\alpha$ in the RL setting. 
% In the first tranfser RL problem, the target MDP's latent factor is $[1, 0]^\top$, the first source MDP's latent factor is $[0, 1]^\top$, and the second source MDP's latent factor is $[1/\alpha, \sqrt{1-1/\alpha^2}]^\top$ for $\alpha \in \R_+$. For large $\alpha$, both source MDPs' latent factors are almost orthogonal to the target MDP's latent factor and makes estimating it with the source MDPs' latent factors very difficult. Thus, $\alpha$ captures the difficulty of using the latent factors from the source MDPs to approximate the target MDP's latent factor. 

Our transfer-ability coefficient is similar to the quantity $\alpha_{\max}$ defined in \cite{agarwal2023provable}. While these terms both quantify the similarity between the source and target MDPs, in our setting, we allow for the source MDPs' state latent factors, $\{F_{m, h}\}$, to differ from target MDP's state latent factors while \cite{agarwal2023provable} assumes that all MDPs share the same latent representation $\phi$. Our setting is more general than the one in \cite{agarwal2023provable} even when assuming the same Tucker rank assumption.

\subsection{Information Theoretic Lower Bound}
To formalize the importance of $\alpha$ in transfer learning, we prove a lower bound that shows that a dependence on $\alpha$ in the sample complexity of the source phase is necessary to improve the regret bound in the target phase. Before proving our main result, we first present an intermediate lower bound to provide intuition on how $\alpha$ measures the difficulty in transferring a learned representation.

\begin{thm}\label{thm:lb_int}
There exists a transfer RL instance that satisfies Assumptions \ref{asm:tr} and \ref{asm:transfer}, in which 
\begin{itemize}[itemsep=0in,topsep=0in]
    \item the learner can only transfer a latent feature representation from a function class $\F$, that contains the true representation, between the source and target phase, and 
    \item the learner cannot change the latent feature representation in the target phase,
\end{itemize}
such that the learner needs to incur a sample complexity $\Omega(\alpha^2)$ in the source MDP to avoid incurring regret $\Omega(T)$ in the target MDP with probability $0.24$. 
\end{thm}
\yccomment{Can we say anything about the dependence on $d,S,A$?}

\yccomment{Can we move the proof to appendix (or replace it with a short proof sketch), and use the space to talk more about the other Tucker rank setting?}
\begin{proof}
Suppose all source and target MDPs $(S, A, P, H, r)$ share the same state space, action space, and horizon $H = 1$ and assume that $S = A = [2n]$ for some $n \in \N_+$. For ease of notation, we let $s_1$ and $a_1$ refer to any state and action in $[n]$, respectively, and $s_2$ and $a_2$ refer to any state and action in $\{n+1, \ldots 2n\}$, respectively.  The initial state distribution in the target MDP is uniform over $S$. We now present two transfer RL problems with similar $Q$ functions (with rows $s_1, s_2$ and columns $a_1,a_2$) that satisfy Assumptions \ref{asm:tr} and \ref{asm:transfer} but have orthogonal target state latent factors. For ease of notation, the superscript $i$ of $Q^{*, i}_{m, h}, Q^{*, i}_{ h}$ denotes transfer RL problem.  Then, the optimal $Q$ functions for transfer RL problem one are
\yccomment{use \texttt{bmatrix} instead of \texttt{tabular} for matrices}
\begin{align*}
    Q^{*, 1}_{1, 1} &= n \begin{bmatrix}
         \sqrt{1/(2n)} \\
          \sqrt{1/(2n)}
    \end{bmatrix}
  \begin{bmatrix}
      \sqrt{1/n} & 0
  \end{bmatrix}= \left[\begin{tabular}{cc}
         $1/\sqrt{2}$ & 0  \\
         $1/\sqrt{2}$ & 0
    \end{tabular} \right],   \quad
    Q^{*, 1}_{1, 2} = n \left[\begin{tabular}{c}
         $\sqrt{1/(2n)}$ \\
          $\sqrt{1/(2n)}$
    \end{tabular} \right] \left[0, \sqrt{1/n} \right] = \left[\begin{tabular}{cc}
         0 & $1/\sqrt{2}$  \\
         0 & $1/\sqrt{2}$
    \end{tabular} \right], \\
    Q^{*, 1}_1 &= n \left[\begin{tabular}{c}
         $\sqrt{1/(2n)}$ \\
          $\sqrt{1/(2n)}$
    \end{tabular} \right] \left[\sqrt{\frac{1}{n}},-\sqrt{\frac{1}{n}} \right] = \begin{bmatrix}
         1/2 & -1/2  \\
         1/2 & -1/2
    \end{bmatrix},
\end{align*}    
and the optimal $Q$ functions for transfer RL problem two are 
\begin{align*}
    Q^{*, 2}_{1, 1} &= n \left[\begin{tabular}{c}
         $\sqrt{1/(2n)}$ \\
          $\sqrt{1/(2n)}$
    \end{tabular} \right] \left[\sqrt{1/n}, 0 \right] = \left[\begin{tabular}{cc}
         $1/\sqrt{2}$ & 0  \\
         $1/\sqrt{2}$ & 0
    \end{tabular} \right],  \quad 
    Q^{*, 2}_{2, 1}  = n F' \left[0, \sqrt{1/n} \right] = \left[\begin{tabular}{cc}
         0 & $(1+1/\alpha)/(c\sqrt{2})$  \\
         0 & $(1-1/\alpha)/(c\sqrt{2})$
    \end{tabular} \right], \\
    Q^{*, 2}_1 &=n \left[\begin{tabular}{c}
         $\sqrt{1/(2n)}$ \\
          $-\sqrt{1/(2n)}$
    \end{tabular} \right] \left[\sqrt{\frac{1}{n}},-\sqrt{\frac{1}{n}} \right] = \left[\begin{tabular}{cc}
         $1/2$ & $-1/2$  \\
         $-1/2$ & $1/2$
    \end{tabular} \right].
\end{align*}
where 
\begin{align*}
F' = \big[&(\sqrt{1/(2n)} + \sqrt{1/(2n\alpha^2})/\sqrt{1 + 1/\alpha^2}, (\sqrt{1/(2n)} - \sqrt{1/(2n\alpha^2})/\sqrt{1 + 1/\alpha^2} \big]^\top.      
\end{align*}
The incoherence $\mu$, rank $d$, and condition number $\kappa$ of the above $Q$ functions are $O(1)$.
Furthermore, the above construction satisfies Assumption \ref{asm:tr} with Tucker rank $(|S|, 1, |A|)$ and Assumption \ref{asm:transfer} because the source and target MDPs share the same state latent factor $[\sqrt{1/(2n)}, \sqrt{1/(2n)}]$ in the first transfer RL problem while in the second transfer RL problem, 
\[
[\sqrt{1/(2n)}, -\sqrt{1/(2n)}] = -\alpha [\sqrt{1/(2n)}, \sqrt{1/(2n)}] + \alpha F^{'\top}.
\]

The learner is given either transfer RL problem one or two with equal probability with a generative model in the source problem. When interacting with the source MDPs, the learner specifies a state-action pair $(s, a)$ and source MDP $m$ and observes a realization of a shifted and scaled Bernoulli random variable $X$. The distribution of $X$ is that $X = 1$ with probability $(Q^{*, i}_{m, 1}(s, a) + 1)/2$ and $X = -1$ with probability $(1 - Q^{*, i}_{m, 1}(s, a))/2)$. Furthermore, the learner is given the knowledge that the state latent features lie in the function class $F = \{ F_1, F_2\}$ and must use the knowledge obtained from interacting with the source MDP to choose one to use in the target MDP, which is no harder than receiving no information about the function class. Finally, the learner is given the target action latent feature $G_T = \left[\sqrt{1/n},-\sqrt{1/n} \right]$. 

To distinguish between the two transfer RL problems, one needs to differentiate between $Q^{*, 1}_{2, 1}$ and $Q^{*, 2}_{2, 1}$. By construction, the magnitude of the largest entrywise difference between $Q^{*, 1}_{2, 1}$ and $Q^{*, 2}_{2, 1}$ is lower bounded by $\Omega(1/\alpha^2)$.
% Note that 
% \begin{align*}
% Q^{*, 2}_2(s_1, a_2) &-  Q^{*, 1}_2(s_1, a_2) = \frac{1/\alpha - 1/\alpha^2}{(1 + 1/\alpha^2)\sqrt{2}} \in \Omega(1/\alpha)\\
% Q^{*, 1}_2(s_s, a_2) &-  Q^{*, 2}_2(s_1, a_2) = \frac{1/\alpha + 1/\alpha^2}{(1 + 1/\alpha^2)\sqrt{2}} \in \Omega(1/\alpha)
% \end{align*}

If the learner observes $Z$ samples in the source MDPs, where $Z \leq C\alpha^2$ for some constant $C > 0$, then the probability of correctly identifying $F$ is upper bounded by $0.76$ \cite{Anthony_Bartlett_1999}. Since the learner is given $G_T$, if the learner chooses $F_1$, their policy always chooses $a_1$. On the other hand, if the learner chooses $F_2$, their policy chooses $a_1$ at $s_1$ and $a_2$ at $s_2$. Thus, by choosing the wrong policy, the learner will incur regret of $2$ at $s_2$, and  $\text{Regret}(T) = \sum_{t\in [T]} V^*(s_t) - V^\pi(s_t) = T$ as the initial state distribution is uniform. It follows that to avoid incurring regret $\Omega(T)$ with probability $0.24$, one must have sample complexity of $\Omega(\alpha^2)$ in the source phase.  
\end{proof}


% Let all source and target MDPs $(S, A, P, H, r)$ share the same state space, action space, and horizon $H = 1$ and assume that $S = A = [2n]$ for some $n \in \N_+$. For ease of notation, we let $s_1$ refer to any state in $[n]$ and $s_2$ refer to any state in $\{n+1, \ldots 2n\}$. Similarly, we let $a_1$ refer to the first half of the actions and let $a_2$ refer to the second half of the actions. The initial state distribution in the target MDP is uniform over $S$. Then, let the state latent factors be $F_1(s_1) = \sqrt{1/(2n)}, F_1(s_2) = \sqrt{1/(2n)}$, $F_2(s_1)= \sqrt{1/(2n)}, F_2(s_2) = -\sqrt{1/(2n)}$, and $F'_1(s_1) = (\sqrt{1/(2n)} + \sqrt{1/(2n\alpha^2})/\sqrt{1 + 1/\alpha^2}, F'_1(s_2) = (\sqrt{1/(2n)} - \sqrt{1/(2n\alpha^2})/\sqrt{1 + 1/\alpha^2}$. We define the action latent factors as $G_1(a_1) = \sqrt{1/n}, G_1(a_2) = 0, G_2(a_1) = 0, G_2(a_2) = \sqrt{1/n},$ $G_T(a_1) = \sqrt{1/(2n)}$, and $G_T(a_2) = -\sqrt{1/(2n)}$. Let $\sigma = n$ be the singular value for all the matrices. Let $c = \sqrt{1 + 1/\alpha^2}$. With these latent factors, we define the $Q$ functions for transfer RL problem one as 
% \begin{align*}
%     Q^{*, 1}_1 &= \sigma F_1 G_1^\top = \left[\begin{tabular}{cc}
%          $1/\sqrt{2}$ & 0  \\
%          $1/\sqrt{2}$ & 0
%     \end{tabular} \right],   \\
%     Q^{*, 1}_2 &= \sigma F_1 G_2^\top = \left[\begin{tabular}{cc}
%          0 & $1/\sqrt{2}$  \\
%          0 & $1/\sqrt{2}$
%     \end{tabular} \right], \\
%     Q^{*, 1}_T &= \sigma F_1 G_T^\top = \left[\begin{tabular}{cc}
%          1/2 & -1/2  \\
%          1/2 & -1/2
%     \end{tabular} \right],
% \end{align*}
% and the $Q$ functions for transfer RL problem two as 
% \begin{align*}
%     Q^{*, 2}_1 &= \sigma F_1 G_1^\top = \left[\begin{tabular}{cc}
%          $1/\sqrt{2}$ & 0  \\
%          $1/\sqrt{2}$ & 0
%     \end{tabular} \right],   \\
%     Q^{*, 2}_2 &= \sigma F' G_2^\top = \left[\begin{tabular}{cc}
%          0 & $(1+1/\alpha)/(c\sqrt{2})$  \\
%          0 & $(1-1/\alpha)/(c\sqrt{2})$
%     \end{tabular} \right], \\
%     Q^{*, 2}_T &=\sigma F_2 G_T^\top = \left[\begin{tabular}{cc}
%          1/2 & -1/2  \\
%          -1/2 & 1/2
%     \end{tabular} \right].
% \end{align*}
% By construction, the incoherence $\mu$, rank $d$, and condition number $\kappa$ in each of the above $Q$ functions are $O(1)$. Furthermore, both transfer learning problems satisfy Assumption \ref{asm:transfer} because $F_2 = -\alpha F_1 + \alpha F'$. 

% To prove our result, we consider the following observation model. The learner is given either transfer RL problem $T_1$ or $T_2$ with equal probability with a generative model in the source problem. Using the generative model to query $Q(s, a)$, the learner observes a realization of a shifted and scaled Bernoulli random variable $X$. The distribution of $X$ is that $X = 1$ with probability $(Q(s, a) + 1)/2$ and $X = -1$ with probability $(1 - Q(s, a))/2)$. Furthermore, the learner is given the knowledge that the state latent features lies in the function class $F = \{ F_1, F_2\}$ and must use the knowledge in the source MDP to choose one to use in the target MDP. Also, the learner cannot switch latent features when in the target phase, and the learner is given access to $G_T$.

% \begin{thm}\label{thm:lb_int}
% Consider the above setting and observation model. Then, one needs to incur a sample complexity $\Omega(\alpha^2)$ in the source MDP to avoid incurring regret $\Omega(T)$ in the target MDP with probability $0.4$. 
% \end{thm}
% \begin{proof}
% To distinguish between the two transfer RL settings, one needs to differentiate $Q^{*, 1}_2$ and $Q^{*, 2}_2$. Note that 
% \begin{align*}
% Q^{*, 2}_2(s_1, a_2) &-  Q^{*, 1}_2(s_1, a_2) = \frac{1/\alpha - 1/\alpha^2}{(1 + 1/\alpha^2)\sqrt{2}} \in \Omega(1/\alpha^2)\\
% Q^{*, 1}_2(s_s, a_2) &-  Q^{*, 2}_2(s_1, a_2) = \frac{1/\alpha + 1/\alpha^2}{(1 + 1/\alpha^2)\sqrt{2}} \in \Omega(1/\alpha^2)
% \end{align*}
% Thus, $\|Q^{*, 1}_2 - Q^{*, 2}_2\|_\infty \in \Omega(1/\alpha)$. If the learner observes $n$ samples in the source MDPs, where $n \leq \frac{9\alpha^2}{50}$, then the probability of the learner correctly identifying $F$ is upperbounded by $0.6$. Since the learner is given $G_T$, if the learner chooses $F_1$, their policy always chooses $a_1$. If the learner chooses $F_2$, their policy chooses $a_1$ at $s_1$ and $a_2$ at $s_2$. Thus, if the learner chooses the incorrect policy $\pi$, the learner will incur regret of $2$ at $s_2$, and  $\text{Regret}(T) = \sum_{t\in [T]} V^*(s_t) - V^\pi(s_t) = T$ as the initial state distribution is uniform. It follows that to avoid incurring regret $\Omega(T)$ with probability $0.4$, one must have sample complexity of $\Omega(\alpha^2)$ in the source phase.  
% \end{proof}


Theorem \ref{thm:lb_int} that one must incur $\Omega(\alpha^2)$ sample complexity on the source MDPs to benefit from transfer learning. However, Theorem \ref{thm:lb_int} forces the learner to choose a state latent factor and use it throughout the whole target phase. We relax this assumption in our main lower bound for this section. 

\begin{thm}\label{thm:lb_tr}
    Let $\F$ be a function class containing the true latent feature representation.
    There exists a transfer RL instance that satisfies Assumptions \ref{asm:tr} and \ref{asm:transfer}  in which the only information the learner can transfer between the source and target phases is a latent feature representation in $\F$. Then, to learn an optimal policy in the target MDP, the learner needs to incur a sample complexity of $\Omega(\alpha^2)$ in the source MDP or $\Omega((|S| + |A|)/\Delta_{\min}^2)$ in the target MDP with probability at least $0.875$.
\end{thm}

Theorem \ref{thm:lb_tr} states that unless one incurs a sample complexity of $\Omega(\alpha^2)$ in the source phase, one cannot remove the dependence on $|S|$ in the target phase. Thus, without incurring some dependence on $\alpha$, one does not benefit from using transfer learning. While Theorem \ref{thm:lb_tr} establishes the necessity of the dependence on $\alpha$ in the source phase, the lower bound on the target MDP is a sample complexity bound instead of a regret bound. Proving a lower bound that states that the learner needs to incur $\Omega(\alpha^2)$ samples in the source phase or incur a regret of $\Omega(\sqrt{|A|T})$ is an interesting open problem. 

The construction used to prove this lower bound is similar to the construction used in the proof of Theorem \ref{thm:lb_int} except we increase the size of the latent feature class. Thus, if the learner does not observe $\Omega(\alpha^2)$ samples in the source phase, then the learner must identify the unique action $a^*$ and then decide on which action (action $a^*$ or action $0$) to choose at each state in the target phase, which results in the dependence on $|S|+|A|$. See Appendix \ref{app:tr_sda} for the formal proof. One can easily prove a similar result in the $(|S|, |S|, d)$ and $(d, |S|, |A|)$ Tucker rank setting with similar constructions by switching the states and actions (see Appendices \ref{app:tr_ssd} and \ref{app:tr_dsa}).  
% One can easily prove a similar result in the $(|S|, |S|, d)$  Tucker rank setting with the same construction by switching the states and actions. 
% Combining the lower bound constructions in the $(|S|, d, |A|)$ and $(|S|, |S|, d)$ Tucker rank settings, we show in Appendix \ref{app:tr_d} that to remove the dependence on both $|S|$ and $|A|$ in the target phase one must incur a source sample complexity of $\Omega(\alpha^4)$.




\tscomment{Should we include a more detailed discussion between the differences between our results and \cite{agarwal2023provable}}
\yccomment{yes}
